Solving nonlinear differential equations on noisy $156$-qubit quantum computers

In this paper, we report on the resolution of nonlinear differential equations using IBM's quantum platform. More specifically, we demonstrate that the hybrid classical-quantum algorithm H-DES successfully solves a one-dimensional material deformation problem and the inviscid Burgers' equation on IBM's 156-qubit quantum computers. These results constitute a step toward performing physically relevant simulations on present-day Noisy Intermediate-Scale Quantum (NISQ) devices.

==> workflow.tex <==
%!TEX root = ../../main-plain.tex
\begin{tikzpicture}[node distance=6cm, scale=.5, every node/.style={scale=0.6}]

\node (input) [action, text width=2.5cm] {{\bf INPUT:}\\ PDEs};

\node (vqc) [action, right of=input, yshift=1.8cm] {\bf VQC};
\node (expval) [action, right of=vqc] {{\bf Expectation values} Function evaluation}; 
\node (bargraph) [right=1mm of expval] {\includegraphics[scale=.25]{bar-graph.png}}; 
\node (pdeseval) [action, below = 1.5cm of expval] {\bf Evaluate PDEs and BCs}; 
\node (loss) [action, left of=pdeseval] {\bf Loss function};
\node (loop) [
  container, 
  right of=input, 
  fit={(vqc) (bargraph) (pdeseval) (loss)},
  xshift=-6cm,
  inner sep=5mm,
  scale=1.6
] {};
\node [above = -2.5mm of loop, label] {\bf HYBRID LOOP};

\node (output) [action, right of=bargraph, yshift=-1.8cm, xshift=-1cm, text width=2.5cm] {{\bf OUTPUT:}\\ Optimal VQC};
% \node (qf-out) [action, xshift=2cm, right of=output] {{\bf OUTPUT:}\\ Solution function};

\draw [arrow] (input) -- (loop);
\draw [arrow] (vqc) -- (expval);
\draw [arrow] (expval) -- (pdeseval);
\draw [arrow] (pdeseval) -- (loss);
\draw [arrow] (loss) -- node[anchor=east] {\bf \textcolor{myblue}{Optimize}} (vqc);
\draw [arrow] (loss) -- node[anchor=west] {\bf \textcolor{myblue}{parameters}} (vqc);
\draw [arrow] (loop) -- (output);
% \draw [arrow] (output) -- node[anchor=south, yshift=3mm] {\bf \textcolor{myblue}{post-processing}} (qf-out);
\end{tikzpicture}

